Communication-Efficient Asynchronous Stochastic Frank-Wolfe over Nuclear-norm Balls

Large-scale machine learning training suffers from two prior challenges, specifically for nuclear-norm constrained problems with distributed systems: the synchronization slowdown due to the straggling workers, and high communication costs. In this work, we propose an asynchronous Stochastic Frank Wolfe (SFW-asyn) method, which, for the first time, solves the two problems simultaneously, while successfully maintaining the same convergence rate as the vanilla SFW. We implement our algorithm in python (with MPI) to run on Amazon EC2, and demonstrate that SFW-asyn yields speed-ups almost linear to the number of machines compared to the vanilla SFW.

==> archiv/1intro_old.tex <==
\section{Introduction}

In this work we tackle the problem of minimizing a convex and smooth function over a trace norm ball:
\begin{equation}
    \min_{\|\bX\|_* \leq \theta} F(\bX) = \frac{1}{N}\sum_i^N f_i (\bX),
\label{eqn:main-problem}
\end{equation}
where $\bX \in \mathbb{R}^{D_1 * D_2}$, and $\|\bX\|_*$ is the trace norm of matrix $\bX$.
This problem formulation covers various important applications, including matrix completion, matrix sensing, multi-label multi-class classification, affine rank minimization, phase retrieval problems, neural network with quadratic activation (see reference therein \cite{allen2017bfw,candes2015phase}). We are especially interested in the case when $D_1, D_2$ are large.

A natural algorithm  in solving Problem \ref{eqn:main-problem} would be the projected gradient descend (PGD) method, which at each iteration computes the gradient and perform a projection onto the trace norm ball. However, the projection requires a full SVD whose complexity is $\mathcal{O}(D_1 D_2 \cdot \min(D_1, D_2))$, and it makes PGD barely applicable in the large scale settings.

To this end, researchers turn their eyes to Frank Wolfe (FW) type methods due to its projection-free nature. At each iteration FW type methods only requires computing the leading left and right singular vectors, and reduces the iteration complexity from $\mathcal{O}(D_1 D_2 \cdot \min(D_1, D_2))$ to $\mathcal{O}(D_1 D_2)$ \cite{allen2017bfw}. The sub-linear convergence rate of FW type methods can either be fixed by properly modifying it as in \cite{allen2017bfw}, or the convergence rate is not of crucial importance as the data provided can be noisy or otherwise limited and hence the statistical error is dominating. 

Due to the exponential growth of the computational requirements and the near-end of Moore's law scaling, there is an increasing interest towards the algorithms that can leverage distributed computational hardwares. FW type mothods are not an exception \cite{zheng2018distributed, bellet2015distributed}. One natural idea to run FW type methods with distributed hardware, is to have a few workers to compute the gradients, and have one master node to aggregate the gradients and compute the update. This approach serves as an competitive baseline in previous arts \cite{zheng2018distributed}. However, there are two challenges: (1) the computation time of each iteration is dominated by the slowest worker, which notoriously hinders the performance of various distributed iterative optimization algorithm \cite{liu2015asynchronous, passcode15, reddi2015variance, recht2011hogwild} (2) the communication cost per iteration is $\Ocal(D_1 D_2)$, which can be unaffordable as $D_1$ and $D_2$ is large.

In this work we try to answer the following two questions:

\textit{ (1) Can FW and FW type algorithms run in an asynchronous (lock-free) manner, so that the iteration time is not dominated by the slowest worker?} 

\textit{ (2) Can we improve the communication cost of running FW in the distributed setting?} 

We answer both of these questions affirmatively, by proposing and analyzing a asynchronous version of Stochastic Frank Wolfe algorithm, which we call \textbf{SFW-asyn}.

\subsection{Our contributions}

\begin{enumerate}
    \item We describe how Stochastic Frank Wolfe algorithm runs asynchronously as in Algo \ref{alg:SFW-asyn} (SFW-asyn). Besides the benefit of not requiring synchronization, SFW-asyn reduces the communication cost from $\Ocal(D_1 D_2)$ as in most existing works, to $\Ocal(D_1 + D_2)$. 
    \item We show the $\mathcal{O}(1/k)$ asymptotic converge rate of Algo \ref{alg:SFW-asyn}, which is in line with the stochastic Frank Wolfe method without asynchrony, as in Theorem \ref{thm:conv-SFW-asyn}.
    \item Besides algorithmic contribution, our analysis framework is generalizable to other Frank Wolfe type method. For example the above results can be extended to Stochastic Variance Reduced Frank Wolfe (SVRF) \cite{hazan2016variance} as in Algo \ref{alg:SVRF-asyn} and Theorem \ref{thm:SVRF-asyn}.
\end{enumerate}

\subsection{Related works}
We mainly overview two different lines of work that is respectively related to distributed Frank-Wolfe algorithm, and asynchronous manner in distributed learning. 
% ADMM?

\textbf{Distributed Frank Wolfe}.

For general network topology, \cite{bellet2015distributed} proposed a distributed Frank Wolfe algorithm for $\ell_1$ and simplex constrain, but not for trace-norm constrained problem. 

On a master-slave computational model, \cite{zheng2018distributed} proposes to distribute the gradient computation among workers and aggregate these gradient by a performing $\Ocal{t}$ distributed power iterations at iteration $t$. This involves even more frequency synchronization than naive distributed Frank Wolfe method  ($\Ocal(T)$ times more where $T$ is the total number of iterations) and will be hindered heavily by staleness. Moreover, to run $T$ iterations, \cite{zheng2018distributed} requires a total communication of $\Ocal(T^2(D_1 + D_2)$, while SFW-asyn only requires $\Ocal(T(D_1 + D_2))$. In the case when the gradients have large spectral gap, \cite{zheng2018distributed} reduces the number of power iterations needed at iteration $t$ to $\Ocal{\log(t)}$. But SFW-asyn still has a great advantages over \cite{zheng2018distributed} due to its asynchronous speedup.

Quantization techniques have also been used to reduce the communication cost for SFW, like \cite{zhang2019quantized}, who proposed a novel gradient encoding scheme (s-partition) to reduce iteration communication cost. However their results are for $\ell_1$ constrained problem, and it is non-trivial to extend their results to trace norm constrained problems. Even if the a similar gradient quantization techniques is invented for Problem \ref{eqn:main-problem}, the communication complexity of quantization based algorithm is still orderwise less competitive than SFW-asyn, as they will required $\Ocal(D_1 D_2)$ bits while SFW-asyn only requires $\Ocal(D_1 + D_2)$ bits.


\textbf{Asynchronous Optimization}. 
There is a rich previous effort in the research on asynchronous optimization, such as asynchronous Stochastic Gradient Descend (SGD) \cite{recht2011hogwild}, asynchronous Coordinate Descend (CD) \cite{liu2015asynchronous, passcode15}, asynchronous Stochastic Variance Reduced Gradient (SVRG) \cite{reddi2015variance}. Mania \textit{et al} proposed a general analysis framework \cite{mania2015perturbed}. However, these analysis approaches cannot be applied to SFW. 
Wang \textit{et al} proposed Asynchronous Block Coordinate FW \cite{wang2014asynchronous} and achieve sub-linear rate. 
They assume that the problem that they are tackling are separable by coordinates, and hence different from our problem setting.
% It follows and extend the algorithms in \cite{lacoste2012block}. 
% Due to its coordinate descend nature, the proof techniques in \cite{lacoste2012block} are directly applicable to \cite{wang2014asynchronous}.

% \textbf{Frank Wolfe Algorithm}.

% \textbf{ADMM}.



% \subsection{Problem and ideas}

% % What about having STORC \cite{hazan2016variance} with asynchronous minibatch (inner loop). Then a linear convergent Asynchronous Frank Wolfe? It will be very interesting to see its ability to handle delay (as asyn-CD is bad at this).

% As SFW requires an increasing batch size, we can consider computing the batch gradient as an inner iteration. The asynchronous idea is to asynchronously computing the inner iteration for SFW and SVRF.

% What kind of error this asyn model introduces? For SFW, the batch gradient may contain a small portion of stochastic gradient calculated based on out-dated $x$. Intuitively, the crux will be bounding the $dist( \nabla f(\bx_k), \nabla f(\bx_{k+1}))$.

% It would be great if we can make our result a framework, as in \cite{mania2015perturbed}.

% % Extend the general framework \cite{reddi2015variance} for non-constrained problem to constrained problem? (then no longer Frank Wolfe). May be trivial by extending the analysis from \cite{reddi2015variance}. If not, check the inexact-GraSP idea. 

==> archiv/_distFW.tex <==
\section*{Convergence of dist-SFW  for vector and $\ell_1 \leq 1$ case.}



\begin{algorithm*}[thb]
{\footnotesize 
\caption{Distributed Inexact Stochastic Frank-Wolfe Method (Dist-SFW)}
\begin{algorithmic}[1]
\FOR{iteration $t=1,2,\cdots, T$}
    \STATE Parameter server send $\bX_t$ to workers.
    \FOR{each worker $w=1,2,\cdots, W$}
        \STATE
        Randomly sample a index set $S_w$ where $|S_w| = m_t/W$
        \STATE Compute $\sum_{i \in S_w} \nabla f_i (\bX_t)$
        \STATE Computing $\bu_w$ and $\bv_w$, the leading left and right singular vector of $-\sum_{i \in S_w} \nabla f_i (\bX_t)$
        \STATE 
        // Note that  $\bu_w \bv_w^T = \argmin_{\|\bU\|_* \leq 1} \quad \langle \sum_{i \in S_w} \nabla f_i (\bX_t), \bU \rangle$ 
        \STATE
        Send $\bu_w$ and $\bv_w$ to the parameter server.
    \ENDFOR
    \STATE
    $\bU_t = (\sum_{w=1}^W \bu_w \bv_w^T)/\| (\sum_{w=1}^W \bu_w \bv_w^T)\|_*$
    \STATE
    $\bX_t \leftarrow \eta_t \bU_t + (1-\eta_t) \bX_{t-1}$
\ENDFOR
% \STATE {\bfseries Output:} $\bx^{(T)}, \by^{(T)}$
\end{algorithmic}
\label{alg:distSFW}}
\end{algorithm*}




\begin{algorithm*}[thb]
{\footnotesize 
\caption{Distributed Inexact Asynchronous Stochastic Frank-Wolfe Method (Dist-Asyn-SFW)}
\begin{algorithmic}[1]
\STATE // The worker algorithm
\FOR{each worker $w=1,2,\cdots, W$}
    \STATE 
    $\bX \leftarrow $ the most recent $\bX_t$ from the parameter server
    \STATE
    Randomly sample a index set $S_w$ where $|S_w| = m_t/W$
    \STATE Compute $\sum_{i \in S_w} \nabla f_i (\bX)$
    \STATE Computing $\bu_w$ and $\bv_w$, the leading left and right singular vector of $-\sum_{i \in S_w} \nabla f_i (\bX)$
    \STATE 
    // Note that  $\bu_w \bv_w^T = \argmin_{\|\bU\|_* \leq 1} \quad \langle \sum_{i \in S_w} \nabla f_i (\bX), \bU \rangle$ 
\ENDFOR
\STATE // The merger algorithm
\FOR{iteration $t=1,2,\cdots, T$}
    \STATE
    Wait until $m_t$ new $\bu_w$ and $\bv_w$ are received.
    \STATE 
    $\bU_t = (\sum_{w=1}^W \bu_w \bv_w^T)/\| (\sum_{w=1}^W \bu_w \bv_w^T)\|_*$
    \STATE
    $\bX_t \leftarrow \eta_t \bU_t + (1-\eta_t) \bX_{t-1}$
    \STATE
    Send $\bX_t$ to the Workers
\ENDFOR
% \STATE {\bfseries Output:} $\bx^{(T)}, \by^{(T)}$
\end{algorithmic}
\label{alg:distAsynSFW}}
\end{algorithm*}

Do this to have an insight of how to show the convergence of nuclear norm problem.

The dist-SFW update would look like the following:
\begin{align}
    &\bu_k = \frac{1}{W} \sum_{w=1}^W \argmin_{\|\bu\|_1 \leq 1} \langle \nabla_w, \bu \rangle \\
    & \bx_k = (1-\eta_k) \bx_{k-1} + \eta_k \bu_k
    \label{eqn:distSFW}
\end{align}
where $\nabla_w$ is the minibatch gradient computed in worker $w$ using $m_k / W$ samples against $\bx_{k-1}$. For the sake of analysis, also define the ground truth update and the worker update:
\begin{align}
   &\bu^* = \argmin_{\|\bu\|_1 \leq 1} \langle \nabla F(\bx_{k-1}), \bu \rangle \\
   & \bu_w = \argmin_{\|\bu\|_1 \leq 1} \langle \nabla_w, \bu \rangle.
   \label{eqn:buw} \\
   & \sigma = \min_{\|\bu\|_1 \leq 1} \langle \nabla F(\bx_{k-1}), \bu \rangle
\end{align}

Note that $\sigma$ is negative.

Then we have
\begin{align*}
    F(\bx_k) & \leq F(\bx_{k-1}) + \langle \nabla F(\bx_{k-1}), \bx_k - \bx_{k-1} \rangle + \frac{1}{2} L \eta_k^2 D^2 \shortrnote{by smoothness} \\
    & = F(\bx_{k-1}) + \eta_k \langle \nabla F(\bx_{k-1}), \bu_k - \bx_{k-1} \rangle + \frac{1}{2} L \eta_k^2 D^2 \shortrnote{by \ref{eqn:distSFW}} \\
    & = F(\bx_{k-1}) + \eta_k \langle \nabla F(\bx_{k-1}), \bu^* - \bx_{k-1} \rangle + \eta_k \langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle +  \frac{1}{2} L \eta_k^2 D^2 \\
    & \leq F(\bx_{k-1}) + \eta_k \langle \nabla F(\bx_{k-1}), \bx^* - \bx_{k-1} \rangle + \eta_k \langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle +  \frac{1}{2} L \eta_k^2 D^2 \\
    & \leq F(\bx^*) + (1-\eta_k)(F(\bx_{k-1}) - F(\bx^*))+ \eta_k \langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle +  \frac{1}{2} L \eta_k^2 D^2 \shortrnote{by convexity}
\end{align*}

Now the focus of the analysis is $\langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle$ and we hope that it decrease at least at the rate of $1/k$ in order to maintain the overall converge rate. 

\vspace{10pt}
\textbf{It seems that $m_k$'s dependence on $W$ (num of workers) is inevitable}

Consider the expectation given $\bx_{k-1}$.
\begin{align*}
    &\expect \langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle \\
    = &\expect \langle \nabla F(\bx_{k-1}), \bu_k\rangle  - \sigma \\
    = &\frac{1}{W}\sum_{w=1}^W \expect \langle \nabla F(\bx_{k-1}), \bu_w\rangle  - \sigma \\
    = &\langle \nabla F(\bx_{k-1}), \expect \bu_w\rangle  - \sigma \shortrnote{Here is the crux}\\
\end{align*}

Or even earlier, before we do the decomposition, let $c = \langle \nabla F(\bx_{k-1}),  \bx_{k-1} \rangle$

\begin{align*}
    &\expect \langle \nabla F(\bx_{k-1}), \bu_k - \bx_{k-1} \rangle \\
    = &\expect \langle \nabla F(\bx_{k-1}), \bu_k\rangle  - c \\
    = &\frac{1}{W}\sum_{w=1}^W \expect \langle \nabla F(\bx_{k-1}), \bu_w\rangle  - c \\
    = &\langle \nabla F(\bx_{k-1}), \expect \bu_w\rangle  - c \shortrnote{Here is the crux}\\
\end{align*}

The convergence depends on $\bu_w$ instead of $\bu_k$, while $\bu_w$ is computed using $m_k / W$ samples. Therefore The co$m_k$ would have to linearly depend on $W$.

\vspace{10pt}
\textbf{what is the goal then?}

For some design of aggregation of $\bu_k$,
\begin{align*}
    \expect \langle \nabla F(\bx_{k-1}), \bu_k\rangle  \leq \sigma + \frac{G}{m_k}
\end{align*}

This seems to be a pure statistical problem. Suppose we have $n$ vectors $\ba_i$ of dimension $d$. We have $W$ workers. They can randomly sample with or without replacement from these $n$ vectors. We can make assumptions about the similarity among $\ba_i$. These workers are only allowed to report a few bits to their master about the minimum index of $\sum \ba_i$. How can the master obtain useful information from all of the workers, so as to estimate the minimum index of $\sum \ba_i$?

\vspace{10pt}
\textbf{With current framework ((1) sample with replacement (2) summation over all workers), this seems to be what we can hope for (sample size depends on $W$ is better than implicitly depends on the dimension)}:
\begin{align*}
    &\langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle \\
    &= \frac{1}{W} \sum_{w=1}^W \langle \nabla F(\bx_{k-1}), \bu_w - \bu^* \rangle \\
    &= \frac{1}{W} \sum_{w=1}^W  \left[\langle \nabla F(\bx_{k-1}) - \nabla_w, \bu_w - \bu^* \rangle + \langle  \nabla_w, \bu_w - \bu^* \rangle \right] \\
    &\leq \frac{1}{W} \sum_{w=1}^W  \langle \nabla F(\bx_{k-1}) - \nabla_w, \bu_w - \bu^* \rangle  \shortrnote{ by \ref{eqn:buw}}\\
    &\leq D \frac{1}{W} \sum_{w=1}^W  \left\| F(\bx_{k-1}) -  \nabla_w \right\| \\
\end{align*}
And take expectation on both side we have
\begin{align*}
\expect \langle \nabla F(\bx_{k-1}), \bu_k - \bu^* \rangle \leq D \frac{G}{\sqrt{m_k/W}}
\end{align*}

Let  $m_k = W \frac{G^2 (k+1)^2}{L^2 D^2}$, $\eta_k = \frac{2}{k+1}$, and we can finish the proof as in standard SFW. But in this analysis, we are essentially allocating $m_k$ samplings for each worker, and therefore no speedup.





==> archiv/_old_6experiment.tex <==
\section{Simulation Results}
\label{sec:simulation}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.45\linewidth]{Figs/sensing_sfw_01/conv.png}
\includegraphics[width=0.45\linewidth]{Figs/sensing_sfw_08/conv.png}
\end{center}
\caption{{\em Convergence performance for the Matrix Sensing problem with various number of workers.} The figures show the relative error decreases over the number of data passes. Simulations are repeated for $10$ times and the range of one standard deviation is shown in the corresponding color shadow (standard deviations are omitted for the first $5$ passes for a clearer view). The staleness model is a geometric distribution with $p=0.1$ for the left plot and $p=0.8$ for the right plot.}
% $\frac{P(\bx^{(t)})-P^*}{P^*}$
\label{fig:convergence} 
\end{figure*}

\begin{figure*}[!thb]
\begin{center}
\includegraphics[width=0.24\linewidth]{Figs/sensing_sfw_01/w4.png}
\includegraphics[width=0.24\linewidth]{Figs/sensing_sfw_01/w8.png}
\includegraphics[width=0.24\linewidth]{Figs/sensing_sfw_01/w16.png}
\includegraphics[width=0.24\linewidth]{Figs/sensing_sfw_08/w4.png}
\end{center}
\caption{Convergence of the relative loss of Matrix Sensing problem VS the time simulated queuing model.}
% $\frac{P(\bx^{(t)})-P^*}{P^*}$
\label{fig:simulated_time} 
\end{figure*}

In this section we empirically show the convergence performance of SFW-asyn and SVRF-asyn, as supported by our theorems. We also show the speedup of SFW-asyn over SFW, and SVRF-asyn over SVRF, under queuing model.

\subsection{Simulation setup}


First let's review two machine learning applications: (1) \textbf{Matrix sensing}. Matrix sensing problem is to estimate a low rank matrix $\bX^*$, with observations of sensing matrices $\bA_i$ and sensing response $y_i = \langle \bA_i, \bX^* \rangle$, for $i = 1...N$. It is an important problem that appears in various fields such as quantun computing, image processing, system design, and so on (see \cite{park2016non} and the reference there in). Its connection to neural network is also an active research topic \cite{li2017algorithmic} (2) \textbf{Polynomial Neural Network (PNN)}. PNN is the neural network with polynomial activation function. PNN has been shown to have universal representation power just as neural networks with sigmoid and relu activation function \cite{livni2014computational}.

We test the performance of SFW-asyn on minimizing the empirical risk of the matrix sensing problem with synthetic data: (1) generate the ground truth matrix $\bX^* = \bU \bV^T / \|\bU \bV^T\|_*$ where $\bU, \bV \in \mathbb{R}^{30*3}$ are generated by uniformly sampling from $0$ to $1$ for each entry; (2) generate $N=900$ sensing matrices $\bA_i$ by sampling each entry from a standard normal distribution (3) compute response $y_i = <\bA_i, \bX^*> + \epsilon$ where $\epsilon$ is sampled from a Gaussian distribution with mean $0$ and variance $0.1$. And hence the empirical risk minimization for this task is
\[
\min_{\|\bX\|_* \leq 1} F(\bX) = \frac{1}{N} \sum_i^N (\langle \bA_i, \bX \rangle - y_i)^2.
\]

We also test SFW-asyn on minimizing the training loss of a Two layers PNN with quadratic activation function and smooth hinge loss to classify MNIST dataset of handwritten digits. In MNIST we have $60000$ training data $(\ba_i, y_i)$, where $\ba_i$ are vectorized $28*28$ pixels images, and $y_i$ are the labels. We set $y_i = -1$ if the label is $0, 1, 2, 3, 4$ or $y_i = 1$ otherwise. We divide the data $\ba_i$ by $255$ therefore they are within zero and one. Hence the training objective of this neural network is
\[
\min_{\|\bX\|_* \leq \theta} F(\bX) = \frac{1}{N} \sum_i^N \textrm{s-hinge}(y_i, \ba_i^T \bX \ba_i),
\]
where the smooth hinge loss function $\textrm{s-hinge}(y, t)$ equals $0.5 - ty$ if $ty \leq 0$,  equals $ (0.5 \cdot (1-ty))^2$ if $0 \leq ty \leq 1$, and equals $0$ otherwise. While one can tune $\theta$ for good classification performance, we only show the results for $\theta=1$ as we are only interested in minimizing the objective value.

In order to better understand how much speedup does asynchrony offer, and the conditions that the speedup occur, we test SFW-asyn against SFW-dist for matrix sensing and PNN under a distributed computational modeled by queuing theory. 

Queuing model is frequently used to model the staleness of each workers in distributed computational setting \cite{mitliagkas2016asynchrony}. We consider each $D_1 D_2$ operation takes one unit of time in expectation. Therefore, each stochastic gradient evaluation of matrix sensing and PNN takes one unit of time in expectation; we solve the 1-SVD up to a practical precision \cite{allen2017bfw}, and we consider 1-SVD takes ten units of time in expectation. In our simulation we find that setting the expected time of 1-SVD as ten or twenty or five has marginal impact on the results. We further assume that the computation time follows a geometric distribution:


For more simulation results and the preliminary simulation results for SVRF-asyn, please checkout our appendix.

\begin{assumption}
Denote random variable $t$ as the computation time required for each worker to finish a computation task that takes $C$ units of time in expectation. Then for $x = C, 2C, ... n C$, $\mathbb{P}(t = x)=p(1-p)^{x/C-1}$ for a distribution parameter $p$.
\end{assumption}

Note that this assumption is \textbf{not required} for our convergence results (Theorem \ref{thm:conv-SFW-asyn} and \ref{thm:SVRF-asyn}) to hold.



\subsection{Convergence of SFW-asyn}


We check how effective SFW-asyn is in using the data. Therefore, we show the relative objective value $(F - F^*)$ against passes of data, as in Fig \ref{fig:convergence}.

One can see from Fig \ref{fig:convergence} that SFW-asyn is almost as effective in using the data as SFW-dist. This means that asynchronous update (using outdated gradient to update $\bX$) has marginal impact on the convergence of the algorithm, render our analysis relatively conservative. This could be due to the nature of the low rank update, or the effect of momentum introduced by asynchrony, as in \cite{mitliagkas2016asynchrony}, and it is an interesting future research direction.

In this result, staleness parameter has marginal impact on the performance of SFW-dist, and the convergence result of SFW-dist is equivalence to SFW. Staleness model does have influence on the performance of SFW-asyn, but as in Fig \ref{fig:convergence}, the impact is marginal.



\subsection{Speedup since asynchronous updates}

\begin{figure}[H]
\begin{center}
\includegraphics[width=0.49\linewidth]{Figs/sensing_sfw_01/speedup.png}
\includegraphics[width=0.49\linewidth]{Figs/sensing_sfw_08/speedup.png}
\end{center}
\caption{Comparing the time needed to achieve the same relative error ($0.03$) against single worker.}
% $\frac{P(\bx^{(t)})-P^*}{P^*}$
\label{fig:simulated_speedup} 
\end{figure}


We show the convergence VS simulated time in Fig \ref{fig:simulated_time}, and the speedup over single worker in in Fig \ref{fig:simulated_speedup}. As in Fig \ref{fig:simulated_speedup}, the speedup of SFW-asyn is almost linear, while SFW-dist compromises as the number of workers get larger.




% \subsection{Speedup due to low communication cost}

% In this section we consider the convergence of the relative loss VS the number of bits being transmitting. We compare SFW-asyn against \cite{zheng2018distributed} since it is the only related work that does not requires $\Ocal{D_1 D_2}$ communication cost. However, we neglect the effect of staleness, which has significant impact on the performance of \cite{zheng2018distributed}, because they requires $\Ocal{t}$ times of synchronization in iteration $t$ and in total $\Ocal(T^2)$ times of synchronization for $T$ iterations, while only $\Ocal(T)$ times of synchronization is needed even for SFW-dist.


==> archiv/_semiasyn.tex <==

\begin{algorithm*}[thb]
{\footnotesize 
\caption{Asynchronous Stochastic Frank-Wolfe Method (SFW-asyn)}
\begin{algorithmic}[1]
% \STATE {\bfseries Input:}  Training data $A\in \mathbb{R}^{n\times d}$, primal and dual step size $\eta,\delta>0$.
\STATE // The worker
\FOR{each worker $w=1,2,\cdots, W$}
    \STATE 
    $\bX \leftarrow $ current $\bX_t$ in the shared memory
    \STATE
    Randomly sample a index set $S_w$ where $|S_w| = m_t/W$
    \STATE compute $\nabla f_i (\bX)$ for $i \in S_w$
    \STATE
    Write the mini-batch gradient in the shared memory
\ENDFOR
\STATE // The parameter server
\FOR{iteration $t=1,2,\cdots, T$}
    \STATE
    Wait until $m_t$ new gradients are computed.
    \STATE 
    $\bU_t \leftarrow \textrm{argmin}_{\|\bU\|_*\leq 1} <\gtil, \bU>$ 
    \STATE
    $\bX_t \leftarrow \eta_t \bU_t + (1-\eta_t) \bX_{t-1}$
    \STATE
    Write $\bX_t$ to the shared memory and cover $\bX_{t-1}$
\ENDFOR
% \STATE {\bfseries Output:} $\bx^{(T)}, \by^{(T)}$
\end{algorithmic}
\label{alg:asynFW}}
\end{algorithm*}


\subsection{Asyn-SFW}
For Asyn-SFW, consider the case when the gradient estimate contains minibatch gradient evaluated on index set $S_1$ against $\bX_{k-1}$, minibatch gradient evaluated on index set $S_2$ against $\bX_{k-2}$, ...  minibatch gradient evaluated on index set $S_\tau$ against $\bX_{k-\tau}$, where $\tau$ is the maximum allowed delay. Note that $\sum_a |S_a| = m_k$. That is,
\[
\gtil_{k} =  \frac{1}{m_k}\sum_{a=1}^{\tau} \left[ 
    \sum_{i \in S_a}  \nabla f_i (\bX_{k-a})
    \right].
\]

We first setup an upper bound for $\langle \nabla F(\bX_{k-1}) - \gtil_{k-1}, \bU_k - \bX^* \rangle$. Then combined with Eq. \ref{eqn:pia} to complete the proof for Theorem \ref{thm:asyn-SFW}.

\begin{lemma}
\jiacheng{TODO}: refine. 
\[
\expect \left [\langle \nabla F(\bX_{k-1}) - \gtil_{k-1}, \bU_k - \bX^* \rangle \right] \leq
\frac{GD}{\sqrt{m_k}} + L \tau \eta_{k-\tau} D^2
\]
\label{lemma:perturb-asyn-SFW}
\end{lemma}
\begin{proof}
\begin{align*}
& \langle \nabla F(\bX_{k-1}) - \gtil_{k-1}, \bU_k - \bX^* \rangle\\
\leq & \|  \nabla F(\bX_{k-1}) - \gtil_{k-1}\|_F \|\bU_k - \bX^*\|_F \\
\leq & D \| \nabla F (\bX_{k-1}) - \gtil_{k-1}\|_F  \\
= & \frac{D}{m_k} \left\lVert m_k\nabla F (\bX_{k-1}) - \sum_{a=1}^{\tau} \left[ \sum_{i \in S_a}  \nabla f_i (\bX_{k-a}) \right]
+ \sum_{a=1}^{\tau}  |S_a|\nabla F (\bX_{k-a}) 
- \sum_{a=1}^{\tau}  |S_a|\nabla F (\bX_{k-a})  \right\rVert \\
= & \frac{D}{m_k} \left\lVert 
    \sum_{a=1}^{\tau} \left [|S_a| \nabla F (\bX_{k-a}) -\sum_{i \in S_a}  \nabla f_i (\bX_{k-a})\right] + 
    \sum_{a=1}^{\tau} |S_a| \left [ \nabla F (\bX_{k-1}) - \nabla F (\bX_{k-a}) \right]
    \right\rVert \\
\leq & \frac{D}{m_k} \left\lVert 
    \sum_{a=1}^{\tau} \left [|S_a| \nabla F (\bX_{k-a}) -\sum_{i \in S_a}  \nabla f_i (\bX_{k-a})\right]
    \right\rVert 
    + \frac{D}{m_k}
    \left\lVert 
    \sum_{a=1}^{\tau} |S_a| \left [ \nabla F (\bX_{k-1}) - \nabla F (\bX_{k-a}) \right]
    \right\rVert 
\end{align*}


Hence now the gradient inexactness is decomposed into two parts: the inexactness resulted from stochastic batch gradient, and the staleness. We increase the batch size and hence obtain a decrease rate of $1/k$ on the first part.
\begin{align*}
    \expect \left [ \sum_{a=1}^{\tau} \left (|S_a| \nabla F (\bX_{k-a}) -\sum_{i \in S_a}  \nabla f_i (\bX_{k-a})\right) \right]^2 \leq {G^2}{m_k},
\end{align*}
and therefore
\begin{align*}
\expect \frac{D}{m_k} \left\lVert 
    \sum_{a=1}^{\tau} \left [|S_a| \nabla F (\bX_{k-a}) -\sum_{i \in S_a}  \nabla f_i (\bX_{k-a})\right]
    \right\rVert
    \leq \frac{GD}{\sqrt{m_k}}
\end{align*}
For the stochastic inexactness, we have to control it by increasing batch size. Note that for some applications when the variance of the stochastic gradient shrinks as the algorithm approach the optimal point, the increasing batch size requirement can be waived.

For the staleness:
\begin{align*}
    &\| \nabla F (\bX_{k-1}) - \nabla F (\bX_{k-\tau}) \|_F \\
    \leq& L \| \bX_{k-1} - \bX_{k-\tau}\|_F \shortrnote{by smoothness}\\
    =& L \| \bX_{k-1} - \bX_{k-2} + \bX_{k-2} + ... - \bX_{k-\tau}\|_F \\
    \leq& L \sum_{a=1}^{\tau+1} \| \bX_{k-a} - \bX_{k-a-1}\|_F \shortrnote{by triangular inequality}\\
    \leq& L \sum_{a=1}^{\tau+1} \eta_{k-a} \| \bU_{k-a} - \bX_{k-a-1}\|_F \shortrnote{by Eq. \ref{eqn:general_fw}}\\
    \leq& L \tau \eta_{k-\tau} D. 
\end{align*}

Therefore 
\begin{align*}
    \sum_{a=1}^{\tau} |S_a| \left [ \nabla F (\bX_{k-1}) - \nabla F (\bX_{k-a}) \right]
    \leq L \tau \eta_{k-\tau} D^2.
\end{align*}
\end{proof}

\textbf{Now we can finish the proof for Theorem \ref{thm:asyn-SFW}}

\begin{proof}
We finish the proof by induction. The case of $k=1$ is trivially true. Suppose $h_k \leq \frac{(2\tau+1)4LD^2}{k+2}$ for $k \leq T-1$. Then
\begin{align*}
h_T \leq &(1-\eta_T) h_{T-1} + \eta_T \left[ \langle \nabla F(\bX_{T-1}) - \gtil_{T-1}, \bU_T - \bX^* \rangle  + \frac{L\eta_T D^2}{2} \right] \\
\leq & (1-\eta_T) h_{T-1} + \eta_T \left[ \frac{GD}{\sqrt{m_T}} + L \tau \eta_{T-\tau} D^2  + \frac{L\eta_T D^2}{2} \right] \shortrnote{by Lemma \ref{lemma:perturb-asyn-SFW}}  \\
= & \frac{T-1}{T+1} h_{T-1} + \frac{2}{T+1} \left[ \frac{LD^2}{T+1} + \frac{2\tau LD^2}{T+1 -\tau}   + \frac{LD^2}{T+1} \right] \shortrnote{plug in $m_T$ and $\eta_T$}  \\
\leq & \frac{T-1}{T+1} \frac{(2\tau+1)4LD^2}{T+1} + \frac{2}{T+1} \left[ \frac{LD^2}{T+1} + \frac{2\tau LD^2}{T+1 -\tau}   + \frac{LD^2}{T+1} \right] \shortrnote{plug in $m_T$ and $\eta_T$}  \\
= & \frac{4LD^2}{(T+1)^2}\left[ (2\tau+1)(T-1) + 1 + \frac{T+1 }{T+1 -\tau}\tau \right]  \\
\leq & \frac{4LD^2}{(T+1)^2}\left[ (2\tau+1)(T-1) + 1 + 2\tau \right]  \shortrnote{$\tau < k/2$}\\
= & \frac{4LD^2}{(T+1)^2}\left[ (2\tau+1)T \right]\\
\leq & \frac{(2\tau+1)4LD^2}{(T+2)}\\
\end{align*} 

\end{proof}
\newpage






==> archiv/_vignette.tex <==

\section{Analysis vignette}

Let's start with a general definition of Frank-Wolfe Method framework.
The update iteration of Frank-Wolfe Method framework is
\[
\begin{split}
    \bs_k &= \argmax_{\bs} \quad \gtil_{k-1}^T \bs \\
    \bx_k &= (1 - \gamma_k) \bx_{k-1} + \gamma_k \bs_k,
\end{split}
\]
where $\gtil$ is the estimate of the gradient at point $\bx_{k-1}$, and $\gamma_k$ is the step size at iterate $k$.
For this framework, let's see how we can analyze it.

Let's assume that the function $f_i$ are convex and $L$-smooth.


\begin{align*}
    f(\bx_k) &\leq f(\bx_{k-1}) + \nabla f (\bx_{k-1})^T (\bx_k - \bx_{k-1}) + \frac{L}{2} \| \bx_k - \bx_{k-1}\|^2  \shortrnote{by smoothness }\\
    &\leq f(\bx_{k-1}) + \gamma_k \nabla f (\bx_{k-1})^T (\bs_k - \bx_{k-1}) + \frac{L\gamma_k^2}{2} \| \bs_k - \bx_{k-1}\|^2 \\
    &\leq f(\bx_{k-1}) + \gamma_k \nabla f (\bx_{k-1})^T (\bs_k - \bx_{k-1}) + \frac{L\gamma_k^2 D^2}{2}
\end{align*}

The third term is very small, as long as we have diminishing step size. Let's look at the second term, which is the focus of our analysis.

\begin{align*}
    &\nabla f (\bx_{k-1})^T (\bs_k - \bx_{k-1})\\
    = & \nabla f (\bx_{k-1})^T (\bs_k - \bx_{k-1}) - \gtil^T (\bs_k - \bx_{k-1})  + \gtil^T (\bs_k - \bx_{k-1}) \\
    \leq & (\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx_{k-1}) + \gtil^T (\bx^* - \bx_{k-1}) \\
    = & \nabla f (\bx_{k-1})^T (\bx^* - \bx_{k-1}) + (\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx^*)  \\
    \leq & f(\bx^*) - f(\bx_{k-1})  + (\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx^*) \\
\end{align*}

Looking good.

\begin{align*}
    f(\bx_k) & \leq  f(\bx_{k-1}) + \gamma_k \left[ f(\bx^*) - f(\bx_{k-1}) + (\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx^*) \right] + \frac{L\gamma_k^2 D^2}{2} \\
    h_k & \leq (1-\gamma_k) h_{k-1} + \gamma_k \left[ (\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx^*) + \frac{L\gamma_k D^2}{2} \right] 
\end{align*}

The last term, we call it residual. Note that if the residual term is zero, then we can have constant step size and achieve linear convergence. Note that $\frac{L\gamma_k D^2}{2}$ comes from a loose bound of $\| x_k - x_{k-1} \|$, which actually diminishes as $k$ gets larger. However let's just live with that and have a loose bound first.

The only remaining term to bound  $(\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx^*)$, which capture the inexactness of the gradient estimation. If the gradient is exact, the proof is then simple. One can plug in $\gamma_k = 2 / (k+1)$ and show by induction that $h(k) \leq 4LD^2 / (k+2)$. Indeed we would like to have this term decrease with the rate of $\mathcal{O}(1/k)$, in order to retain the $\mathcal{O}(1/k)$ convergence rate (easy to show).

Now let's consider the case when $\gtil$ contains $S_1$ samples of $f_i(\bx_{k-1})$, $S_2$  samples of $f_i(\bx_{k-2})$, ...  $S_t$  samples of $f_i(\bx_{k-t})$, where $t$ is the maximum allowed delay.

\begin{align*}
& (\nabla f (\bx_{k-1}) - \gtil)^T (\bs_k - \bx^*) \\
\leq & \| \nabla f (\bx_{k-1}) - \gtil\| \|\bs_k - \bx^*\| \\
\leq & D \| \nabla f (\bx_{k-1}) - \gtil\|  \\
= & D \| \nabla f (\bx_{k-1}) - \gtil + \sum_{a=2}^t \frac{S_a}{S}\nabla f (\bx_{k-a}) - \sum_{a=2}^t \frac{S_a}{S} \nabla f (\bx_{k-a}) \| \\
= & D \left\lVert 
    \sum_{a=a}^t \left [\frac{S_a}{S}\nabla f (\bx_{k-a}) - \frac{1}{S}\sum_{i=1}^{S_a} \nabla f_i(\bx_{k-a})\right] + 
    \sum_{a=2}^t \left [ \frac{S_a}{S} \nabla f(\bx_{k-1}) - \frac{S_a}{S} \nabla f (\bx_{k-a}) )\right]
    \right\rVert \\
\leq & D \left\lVert 
    \sum_{a=a}^t \left [\frac{S_a}{S}\nabla f (\bx_{k-a}) - \frac{1}{S}\sum_{i=1}^{S_a} \nabla f_i(\bx_{k-a})\right] 
    \right\rVert
    +
    D \left\lVert
    \sum_{a=2}^t \left [ \frac{S_a}{S} \nabla f(\bx_{k-1}) - \frac{S_a}{S} \nabla f (\bx_{k-a}) )\right]
    \right\rVert
\end{align*}

Hence now the gradient inexactness is decomposed into two parts: the inexactness resulted from stochastic batch gradient, and the delay. We increase the batch size and hence obtain a decrease rate of $1/k$ on the first part.


\begin{align*}
    &\| \nabla f(\bx_{k-1}) - \nabla f (\bx_{k-2}) \| \\
    \leq& L \| \bx_{k-1} - \bx_{k-2}\| \\
    \leq& L \gamma_{k-1} \| \bs_{k-1} - \bx_{k-2}\| \\
    \leq& L \gamma_{k-1} D,
\end{align*}
which decrease at the rate of $1/k$.

\subsection{Consider the conflict graph as in Hogwild!?}

The conflict graph is not suitable for the analysis of SFW. SFW require increasing batchsize as we approaching the optimal point, and increasing batch-size means increasing average degree (probabiliy of conflict), as in the conflict graph model in Hogwild!. One could definitely encode the average degree as an increasing sequence with respect to the iteration number $k$, but that would lead to a cumbersome analysis, and having a sequence of parameters that hard to quantify in practise. 

Due to similar reason, we assume that the reading operation is also atomic.



==> archiv/deleted <==
{\color{red} the following is what I meant for block frank-wolfe with linear convergence under distributed setting  }
\section{Synchronous Frank-Wolfe with Linear Convergence}
\begin{assumption}
Each batch shares a same minimizer $\bx^*$:
\begin{equation*}
    f_i(\bx^*) = \min_{\|\bx\|_1\leq \tau } f_i(\bx). 
\end{equation*}
Here $f_i$ is the function loss on the $i$-th machine. $\bx^*$ is at most $s$-sparse. 
\end{assumption}
\begin{theorem}
Distributed Block Frank-Wolfe yields linear convergence rate and only requires to communicate a $s$-sparse vector from each worker to the parameter server. 
\label{thm:syn_BFW}
\end{theorem}
\begin{proof}[Proof of Theorem \ref{thm:syn_BFW}]
For each worker $i$, we compute the potential update direction $\tilde{\bx}^{(i)} $ that is $s-$sparse:
\begin{equation*}
    \tilde{\bx}^{(i)} \leftarrow \min_{\bx} \left\{\langle \nabla f_i(\bx_{t-1}),\bx\rangle + \frac{L}{2}\eta \|\bx_{t-1}-\bx\|^2 \right\}
\end{equation*}
When we aggregate as the parameter server, we have $\bx_t\leftarrow \bx_{t-1}+\eta \frac{1}{n}\sum_{i=1}^n (\tilde{\bx}^{(i)}-\bx_{t-1})$. 
Notice
\begin{eqnarray*}
\sum_i \langle \nabla f_i(\bx_{t-1}), 
\end{eqnarray*}


With similar argument as our paper \cite{lei2019primal}, we have:

$f_i(\bx_{t-1}+\eta(\tilde{\bx}^{(i)}-\bx_{t-1}))-f^*_i\leq (1-1/4\kappa)(f_i(\bx_{t-1})-f^*_i)$. 


Therefore we have:
\begin{eqnarray*}
&&f(\bx_t)-f^*\\
&=& \sum_{i=1}^n f_i(\bx_t) -f_i^* \\
&& 
\end{eqnarray*}



\end{proof}
